Towards Deeper Understanding of Variational Autoencoding Models

We propose a new family of optimization criteria for variational auto-encoding models, generalizing the standard evidence lower bound. We provide conditions under which they recover the data distribution and learn latent features, and formally show that common issues such as blurry samples and uninformative latent features arise when these conditions are not met. Based on these new insights, we propose a new sequential VAE model that can generate sharp samples on the LSUN image dataset based on pixel-wise reconstruction loss, and propose an optimization criterion that encourages unsupervised learning of informative latent features.

==> abstract.tex <==
% We propose a family of optimization criteria for
% variational auto-encoding methods under a motivation, of which the well known evidence lower bound (ELBO) is a special case. 
% Under this novel derivation we are able to both formally and intuitively explain when and why VAE is successful or unsuccessful. We also propose several methods to improve VAE models based on our new insight, and open up several new questions whose solution has the potential of significantly improving VAE styled models.

% We propose a new sequential VAE model that can generate sharp samples on complex image datasets. 

We propose a new family of optimization criteria for
variational auto-encoding models, generalizing the standard evidence lower bound. 
%Even though they are not always lower bounds on the margina likelihood, 
We provide conditions under which they recover the data distribution and learn latent features, and formally show that common issues such as blurry samples and uninformative latent features arise when these conditions are not met.
%provide new insights into 
%common failure modes of existing VAE techniques.
Based on these new insights, we propose a new sequential VAE model that can generate sharp samples on the LSUN image dataset based on pixel-wise reconstruction loss, 
%. We also 
and propose an optimization criterion that encourages unsupervised learning of informative latent features.



==> cmds.tex <==
\usepackage{hyperref}
\usepackage[english]{babel}
\usepackage{url}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{wrapfig}
\usepackage{bm}
\usepackage{psfrag}
\usepackage{tikz}
\usepackage{epstopdf}
\usepackage{adjustbox}

\newcommand{\beq}[1][\vspace{0.3em}]{#1\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\rbx}[2][!]{
	\resizebox{#1}{!}{$#2$}	
}
\newcommand{\eqs}[1]{\begin{align}#1\end{align}}
\newcommand{\mat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bit}{\vspace{0mm}\begin{itemize}}
\newcommand{\eit}{\vspace{0mm}\end{itemize}}
\newcommand{\ben}{\vspace{0mm}\begin{enumerate}}
\newcommand{\een}{\vspace{0mm}\end{enumerate}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}

\newcommand{\Av}[0]{{{\bf A}}}
\newcommand{\Bv}[0]{{{\bf B}}}
\newcommand{\Cv}[0]{{{\bf C}}}
\newcommand{\Dv}[0]{{{\bf D}}}
\newcommand{\Ev}[0]{{{\bf E}}}
\newcommand{\Fv}[0]{{{\bf F}}}
\newcommand{\Gv}[0]{{{\bf G}}}
\newcommand{\Hv}[0]{{{\bf H}}}
\newcommand{\Iv}[0]{{{\bf I}}}
\newcommand{\Jv}[0]{{{\bf J}}}
\newcommand{\Kv}[0]{{{\bf K}}}
\newcommand{\Lv}[0]{{{\bf L}}}
\newcommand{\Mv}[0]{{{\bf M}}}
\newcommand{\Nv}[0]{{{\bf N}}}
\newcommand{\Ov}[0]{{{\bf O}}}
\newcommand{\Pv}[0]{{{\bf P}}}
\newcommand{\Qv}[0]{{{\bf Q}}}
\newcommand{\Rv}[0]{{{\bf R}}}
\newcommand{\Sv}[0]{{{\bf S}}}
\newcommand{\Tv}[0]{{{\bf T}}}
\newcommand{\Uv}[0]{{{\bf U}}}
\newcommand{\Vv}[0]{{{\bf V}}}
\newcommand{\Wv}[0]{{{\bf W}}}
\newcommand{\Xv}[0]{{{\bf X}}}
\newcommand{\Yv}[0]{{{\bf Y}}}
\newcommand{\Zv}[0]{{{\bf Z}}}

\newcommand{\av}[0]{{{\bf a}}}
\newcommand{\bv}[0]{{{\bf b}}}
\newcommand{\cv}[0]{{{\bf c}}}
\newcommand{\dv}[0]{{{\bf d}}}
\newcommand{\ev}[0]{{{\bf e}}}
\newcommand{\fv}[0]{{{\bf f}}}
\newcommand{\gv}[0]{{{\bf g}}}
\newcommand{\hv}[0]{{{\bf h}}}
\newcommand{\iv}[0]{{{\bf i}}}
\newcommand{\jv}[0]{{{\bf j}}}
\newcommand{\kv}[0]{{{\bf k}}}
\newcommand{\lv}[0]{{{\bf l}}}
\newcommand{\mv}[0]{{{\bf m}}}
\newcommand{\nv}[0]{{{\bf n}}}
\newcommand{\ov}[0]{{{\bf o}}}
\newcommand{\pv}[0]{{{\bf p}}}
\newcommand{\qv}[0]{{{\bf q}}}
\newcommand{\rv}[0]{{{\bf r}}}
\newcommand{\sv}[0]{{{\bf s}}}
\newcommand{\tv}[0]{{{\bf t}}}
\newcommand{\uv}[0]{{{\bf u}}}
\newcommand{\vv}[0]{{{\bf v}}}
\newcommand{\wv}[0]{{{\bf w}}}
\newcommand{\xv}[0]{{{\bf x}}}
\newcommand{\yv}[0]{{{\bf y}}}
\newcommand{\zv}[0]{{{\bf z}}}
\newcommand{\epsilonv}[0]{{{\bf \epsilon}}}

\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\mb}[1]{\mbox{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}

\providecommand{\abs}[1]{\,\lvert#1\rvert\,}
\providecommand{\norm}[2]{\,\lVert#1\rVert_#2 \,}
\newcommand{\Var}{\operatorname{Var}}

\providecommand{\tightlist}{%
	\setlength{\itemsep}{2pt}\setlength{\parskip}{2pt}}

\providecommand{\js}[1]{{\color{red} [JS: #1]}}
\providecommand{\shengjia}[1]{{\color{blue} [SJ: #1]}}

==> introduction.tex <==
\section{Introduction}

%Generative modeling seeks to model the joint distribution $p_{data}(x)$ for unlabeled data with an approximating distribution $p_\theta(x)$. 

%Recent advances with generative modeling enable us to model the distribution over complex natural datasets
Generative models have made remarkable progress in recent years. Existing techniques can model fairly complex datasets, including natural images and speech~\citep{deconvolutional_gan2015, wgan2017, pixel_rnn2015, conditional_pixelcnn2016, infusion_training2016, vae_autoregressive_flow2016, pixel_vae2016, generate_text2015, recurrent_vae_sequence2015}. %\stefano{add a few more. chemistry, bio, maybe NLP }\shengjia{Added some NLP. I'm not aware of bio or chem papers}
Latent variable models, such as variational autoencoders (VAE), are among the most successful ones. 
%\stefano{explicitly model latent variables to capture latent factors of variation. can be used for unsupervised feature learning}
%\stefano{flexible generative model parameterized using neural networks. flexible but posterior is intractable, and learning is hard.}
%\stefano{solution is to jointly train an inference network to approximate the posterior. joint variational optimization problem}
\citep{autoencoding_variational_bayes2013, variational_dbn_stochastic_bp2014, vae_autoregressive_flow2016, ladder_variational_network2015, matnet_variational_network2016, pixel_vae2016}. 
%This class of models seek to explicitly capture the latent factors of variations through unobserved latent variables. 
%The model usually specifies a simple prior on latent variables, and a conditional distribution of observed variables given latent variables. The conditional distribution is often represented by a parameterized deep network.
These generative models are very flexible, but
%posterior inference over the latent variables and learning is generally intractable. 
the resulting marginal likelihood 
%over the observed data 
is intractable to compute and optimize.
%, making learning difficult. 
Models are thus learned by optimizing a tractable "evidence lower bound", obtained using a tunable inference distribution.
%The solution is to jointly train an inference distribution that is also represented by a deep network, and optimize a variational optimization problem to learn both the generative distribution and approximate inference distribution. 

Despite the empirical success, 
%several problems remain to be solved. First, 
existing VAE models are unable to accurately model complex, large scale image datasets such as LSUN and Imagenet, unless other approaches such as adversarial training or supervised features are employed \citep{generative_network_perceptual_metric2016, autoencoder_with_gan_metric2015, discriminative_reg_for_vae2016}. 
When applied to complex datasets of natural images, VAE models tend to produce unrealistic, blurry samples
%The common mode of failure for these difficult datasets is the generation of visually fuzzy samples
\citep{generative_network_perceptual_metric2016}. The sample quality can be improved with a more expressive generative model, however, 
%in that case there is 
this leads to
a tendency to ignore the latent variables, thus 
hindering the unsupervised feature learning goal
%preventing learning
%A second commonly observed problem is the inability to use the latent variables in a way that leads to 
%useful features for unsupervised learning 
\citep{lossy_vae2016}. 
%where the model ignores the latent code and uses the same conditional distribution to model data whatever value latent variables take. 
%This fails to learn a latent factors or features which is often a major purpose of unsupervised learning.
%It is important that we gain deeper understanding into the properties of VAE models so that we can develop solutions that target these problems. 

In this paper, we propose a new derivation of VAEs which is not based on a variational Bayes approach.
%. It is not based on variational approximation of the (intractable) posterior of a latent variable generative model $p(x|z)$,
%but instead on variational approximation of the (intractable) posterior of a feature detector $q(z|x)$. 
We propose a new and more general optimization criterion that is not always a lower bound on the marginal likelihood, but it is guaranteed to learn the data distribution under suitable conditions. For a particular choice of regularization, our approach becomes the regular VAE \citep{autoencoding_variational_bayes2013}.
%This paper makes the following contributions. In section 2 we derives VAE models under a different motivation, and give a new perspective to understanding the workings of VAE models. 
This new derivation gives us insights into the properties of VAE models. In particular, we are able to formally explain some common failure modes of VAEs, and propose novel methods to alleviate these issues.

In Section 3 we provide a formal explanation for why VAEs generate blurry samples when trained on complex natural images. We show that under some conditions, blurry samples are not caused by the use of a maximum likelihood approach as previously thought, but rather they are caused by an inappropriate choice for the inference distribution.
%only a special case of a more general problem caused by badly learned feature detectors. 
We specifically target this problem by proposing a sequential VAE model, where we gradually augment the the expressiveness of the inference distribution using a process %similar in spirit to 
inspired by
the recent infusion training process\citep{infusion_training2016}.
%quality of latent features. 
As a result, we are able to generate sharp samples on the LSUN bedroom dataset, even using $2$-norm reconstruction loss in pixel space.

In Section 4 we propose a new explanation of the VAE tendency to ignore the latent code. We show that this problem is specific to the original VAE objective function \citep{autoencoding_variational_bayes2013} and does not apply to the more general family of VAE models we propose. We show experimentally that using our more general framework, we achieve comparable sample quality as the original VAE, 
while at the same time learning meaningful features through the latent code,
%taking advantage of the latent code,
%and can place a significant amount of information into the latent code 
even when the decoder is a powerful PixelCNN that can by itself model data \citep{pixel_rnn2015, conditional_pixelcnn2016}. 
%More importantly we point to the right questions to ask when we want to further alleviate or even, solve, these problems.







==> latent.tex <==
Let $p_{data}(x)$ be the true underlying data distribution defined over $x \in \mathcal{X}$, and $\mathcal{D}$ be a dataset of i.i.d. samples from $p_{data}(x)$. 
In the context of unsupervised learning, we are often interested in learning features and representations directly from unlabeled data. A common approach for inducing features is to consider a joint probability distribution $p(x,z)$ over $(x,z)$, where $x \in \mathcal{X}$ is in the observed data space and $z \in \mathcal{Z}$ is a {\em latent code} or {\em feature space}. The distribution $p(x,z)$ is specified with a prior $p(z)$ and a conditional $p(x|z)$. The prior $p(z)$ is often chosen to be relatively simple -- the hope is that the interactions between high level features are disentangled, and can be well approximated with a Gaussian or  uniform distribution. The complexity of $p_{data}(x)$ is instead captured by the conditional distribution $p(x|z)$. For the analysis in this paper, it will be convenient to specify $p(x|z)$ using two components:

%First we formally define latent variable models and the notations we will use throughout the paper. 
\begin{enumerate}
\item A family of probability distributions $\mathcal{P}$ over $\mathcal{X}$. We require that the set $\mathcal{P}$ is parametric, which means that it can be indexed by a set $\Lambda$ in finite dimensional real space $\Lambda \subset \mathbb{R}^D$. We furthermore require that for every $\lambda \in \Lambda$, the corresponding element $\mathcal{P}_\lambda$ has well-defined and tractable log likelihood derivative $\nabla_\lambda \log \mathcal{P}_\lambda(x)$ for any $x \in \mathcal{X}$. 
%This requirement is satisfied for elementary distributions such as non-singular Gaussians \citep{autoencoding_variational_bayes2013} \citep{variational_dbn_stochastic_bp2014} where $\Lambda = \lbrace \lambda = (\mu, \Sigma)| \mu \in \mathbb{R}^N, \Sigma \in \mathbb{S}_N^+$, where $\mathbb{S}_n^+$ are positive definite matrices, and the mapping $\mathcal{P}_\lambda = \mathcal{N}(\mu, \Sigma)$, or the family of recurrent density estimators \citep{pixel_vae2016}, where $\mathcal{P}_\lambda(x) = \prod_{i=0}^{N} p_\lambda(x_i|x_{<i})$, and $p_\lambda$ is a neural network parameterized by $\lambda$. 
\item A mapping $f_\theta: \mathcal{Z} \to \Lambda$ parameterized by $\theta$ with well defined and tractable derivatives $\nabla_\theta f_\theta(z)$ for all $z \in \mathcal{Z}$. We also denote the family of all possible mappings defined by our model as $\mathcal{F}=\{f_\theta, \theta \in \Theta\}$. 
%In practice $\mathcal{F}$ is often a deep neural network
\end{enumerate}

Given $\mathcal{P}$ and $\mathcal{F}$, we define a family of models
\[ p_\theta(x, z) = p_\theta(x|z) p(z) = \mathcal{P}_{f_\theta(z)}(x)p(z) \]
indexed by $\theta \in \Theta$. Note that $ \mathcal{P}_{f_\theta(z)}$ plays the role of the conditional distribution $p_\theta(\cdot \mid z)$ for any given $z \in \mathcal{Z}$. For brevity, we will use $p_\theta(x|z)$ to indicate $\mathcal{P}_{f_\theta(z)}(x)$. Note that the resulting marginal likelihood $p_\theta(x)$ is a mixture of distributions in $\mathcal{P}$
\[ p_\theta(x) = \int_z p(z) p_\theta(x|z) dz = \E_{p(z)}[p_\theta(x|z)] \]

While the specification of $p_\theta(\cdot | z)$ using $\mathcal{P}$ and $f_\theta$ is fully general, our definition imposes some (mild) tractability restrictions on $\mathcal{P}$ and $f_\theta$ to allow for efficient learning. Specifically, the models we consider are those where 
$\nabla_\theta p_\theta(x|z)$ can be tractably computed using the chain rule: 
\[ \nabla_\theta p_\theta(x|z) = \frac{\partial \log \mathcal{P}_{\lambda}(x)}{\partial \lambda}^T \frac{\partial \lambda}{\partial \theta} = \frac{\partial \log \mathcal{P}_{\lambda}(x)}{\partial \lambda}^T \frac{\partial f_\theta(z)}{\partial \theta} \] 
This class of models encompasses many recent approaches~\citep{autoencoding_variational_bayes2013, vae_autoregressive_flow2016, conditional_pixelcnn2016, pixel_vae2016}, where $\mathcal{P}$ is often Gaussian or a recurrent density estimator, and $\mathcal{F}$ is a deep neural network.
%Other models such as non-parametric models are possible but beyond the scope of this paper.
%\stefano{show that this is fully general} \shengjia{The original formulation seems to be lack the newly added technical detail, and are not fully general}\stefano{it seems that a lot of the results hold generally. e.g., we only need derivatives to optimize efficiently, but for other results, it's fine}

We consider a maximum likelihood based approach to learn the parameters, where the goal is to maximize the marginal likelihood of the data
\begin{align*}
\max_\theta &\E_{p_{data}(x)}[\log p_\theta(x)] \\ 
&= \max_{\theta} \E_{p_{data}(x)} \left[\log \E_{p(z)}[p_\theta(x|z)] \right] \numberthis \label{equ:maximum_likelihood}
\end{align*}
%\stefano{combine equations to save space}
where the expectation over $p_{data}(x)$ is approximated using a sample average over the training data $\mathcal{D}$.

%\stefano{objective is non-convex. even finding a local optimum by gradient descent can be hard.}
To actually optimize over the above criteria we require that for any $x$, the derivative over model parameters of $\nabla_\theta \log p_\theta(x)$ be easy to compute or estimate. However tractability of $\nabla_\theta p_\theta(x|z)$ do not imply tractability of $\nabla_\theta p_\theta(x)$, and if we directly take the derivative we get
\begin{align*}
\nabla_\theta \log p_\theta(x) &= p_\theta(x)^{-1} \nabla_\theta E_{p(z)}[p_\theta(x|z)] \\ 
&= p_\theta(x)^{-1} E_{p(z)}[\nabla_\theta p_\theta(x|z)] \numberthis \label{equ:intractable_model}
\end{align*}
Evaluating $p_\theta(x)^{-1}$ involves the computation of a high dimensional integral. Even though this integral can be approximated by sampling 
\[ p_\theta(x) = E_{p(z)}[p_\theta(x|z)] \approx \frac{1}{n} \sum_{z_i, \cdots, z_n \sim p(z)} p_\theta(x|z_i) \]
this costly approximation has to be performed for every sample $x \sim p_{data}(x)$.
%\stefano{try to make this last paragraph more precise if possible}



%\stefano{might be cleaner to use $\E_{x \sim p_{data}}$ instead of $\E_{p_{data}(x)}$}

%\stefano{this notation $f_\theta(z)(x)$ is very confusing}

%\stefano{note: probability distribution vs prob density}

==> oldintro.tex <==
Let $p_{data}(x)$ be the true underlying data distribution defined over $x \in \mathcal{X}$. Let $p_\theta(x)$ be a family of distributions parameterized by $\theta \in \Theta$. The maximum likelihood estimate of the parameters $\theta^*$ is obtained by maximizing
\begin{align*}
\max_\theta \E_{p_{data}(x)}[\log p_\theta(x)] \numberthis \label{equ:maximum_likelihood}
\end{align*}
Several classes of models have been devised to perform this density estimation task directly, usually with a recurrent or auto-regressive structure \citep{pixel_rnn2015} \citep{masked_autoregressive_autoencoder2015} \citep{deep_autoregressive_network2013}. However, in the context of unsupervised learning we  often want to learn meaningful features and representations from unlabeled data.
%, so that they can benefit down-stream tasks of supervised learning or reinforcement learning where we labels/samples are expensive.


A common approach for inducing features is to introduce a joint probability distribution $p(x,z)$ over $(x,z)$, where $x \in \mathcal{X}$ is in the observed data space and $z \in \mathcal{Z}$ is a latent code or feature space. The distribution $p(x,z)$ is specified with a prior $p(z)$ and a conditional $p(x|z)$. The prior $p(z)$ is often simple -- the hope is that the interaction between high level features is simple and disentangled, so that it can be described with some simple prior such as $\mathcal{N}(0, I)$ or a uniform distribution on a convex set. We place the complexity instead into the conditional distribution $p(x|z)$. The conditional distribution actually contains two parts, which we will later show to have very different consequences for model performance. The two parts are defined as follows
\begin{enumerate}
\item A distribution family $\mathcal{P}$, which we suppose to be fixed a-priori by the model class we choose. We require that the set $\mathcal{P}$ is parametric, which means that it can be indexed by a set $\Lambda$ in finite dimensional real space $\Lambda \subset \mathbb{R}^D$. We furthermore require that for every $\lambda \in \Lambda$, the corresponding element $\mathcal{P}_\lambda$ has well-defined and tractable log likelihood derivative $\nabla_\lambda \log \mathcal{P}_\lambda(x)$ for any $x \in \mathcal{X}$. This requirement is satisfied for elementary distributions such as non-singular Gaussians \citep{autoencoding_variational_bayes2013} \citep{variational_dbn_stochastic_bp2014} where $\Lambda = \lbrace \lambda = (\mu, \Sigma)| \mu \in \mathbb{R}^N, \Sigma \in \mathbb{S}_N^+$, where $\mathbb{S}_n^+$ are positive definite matrices, and the mapping $\mathcal{P}_\lambda = \mathcal{N}(\mu, \Sigma)$, or the family of recurrent density estimators \citep{pixel_vae2016}, where $\mathcal{P}_\lambda(x) = \prod_{i=0}^{N} p_\lambda(x_i|x_{<i})$, and $p_\lambda$ is a neural network parameterized by $\lambda$. 
\item A mapping $f_\theta: \mathcal{Z} \to \Lambda$ parameterized by $\theta$ with well defined and tractable derivatives $\nabla_\theta f_\theta(z)$ for all $z \in \mathcal{Z}$. We also denote the family of all possible mappings defined by our model as $\mathcal{F}=\{f_\theta, \theta \in \Theta\}$. In practice $\mathcal{F}$ is often a deep neural network
\end{enumerate}

Given $\mathcal{P}$ and some mapping $f_\theta$ we fully specify the joint distribution of the model
\[ p_\theta(x, z) = p_\theta(x|z) p(z) = \mathcal{P}_{f_\theta(z)}(x)p(z) \]
To avoid cluttering the notation we shall use $p_\theta(x|z)$ rather than the decomposed notation unless we are directly referring to $\mathcal{P}$ or $f$. 

Note that this does not account for all latent variable models. But it accounts for those where $\nabla_\theta p_\theta(x|z)$ can be tractably computed by back propagation. 
\[ \nabla_\theta p_\theta(x|z) = \frac{\partial \log \mathcal{P}_{\lambda}(x)}{\partial \lambda}^T \frac{\partial \lambda}{\partial \theta} = \frac{\partial \log \mathcal{P}_{\lambda}(x)}{\partial \lambda}^T \frac{\partial f_\theta(z)}{\partial \theta} \] 
This class of models account for most recent advances in generative modeling. (cite some examples) Other models such as non-parametric models are possible but beyond the scope of this paper.
%\stefano{show that this is fully general} \shengjia{The original formulation seems to be lack the newly added technical detail, and are not fully general}\stefano{it seems that a lot of the results hold generally. e.g., we only need derivatives to optimize efficiently, but for other results, it's fine}

We can rewrite our original model as a mixture of distributions in $\mathcal{P}$
\[ p_\theta(x) = \int_z p(z) p_\theta(x|z) dz = \E_{p(z)}[p_\theta(x|z)] \]
and our optimization can be written in a similar form
\begin{align*}
\max_{\theta} \E_{p_{data}(x)} [\log E_{p(z)}[\log p_\theta(x|z)] ] \numberthis \label{equ:original_expanded_criteria}
\end{align*}
To actually optimize over the above criteria we require that for any $x$, the derivative over model parameters of $\nabla_\theta \log p_\theta(x)$ be tractable, or at least have a low variance estimator. However tractability of $\nabla_\theta p_\theta(x|z)$ do not imply tractability of $\nabla_\theta p_\theta(x)$, and if we directly take the derivative we get
\begin{align*}
\nabla_\theta \log p_\theta(x) &= p_\theta(x)^{-1} \nabla_\theta E_{p(z)}[p_\theta(x|z)] \\ 
&= p_\theta(x)^{-1} E_{p(z)}[\nabla_\theta p_\theta(x|z)] \numberthis \label{equ:intractable_model}
\end{align*}

Evaluating $p_\theta(x)^{-1}$ involves the computation of a high dimensional integral. Even though this integral can be approximated by sampling, this approximation is costly and has to be performed for every sample $x \sim p_{data}(x)$. 
